Emergent Communication for Rules Reasoning

Research on emergent communication between deep-learning-based agents has received extensive attention due to its inspiration for linguistics and artificial intelligence. However, previous attempts have hovered around emerging communication under perception-oriented environmental settings, that forces agents to describe low-level perceptual features intra image or symbol contexts. In this work, inspired by the classic human reasoning test (namely Raven's Progressive Matrix), we propose the Reasoning Game, a cognition-oriented environment that encourages agents to reason and communicate high-level rules, rather than perceived low-level contexts. Moreover, we propose 1) an unbiased dataset (namely rule-RAVEN) as a benchmark to avoid overfitting, 2) and a two-stage curriculum agent training method as a baseline for more stable convergence in the Reasoning Game, where contexts and semantics are bilaterally drifting. Experimental results show that, in the Reasoning Game, a semantically stable and compositional language emerges to solve reasoning problems. The emerged language helps agents apply the extracted rules to the generalization of unseen context attributes, and to the transfer between different context attributes or even tasks.

==> sections/introduction-old.tex <==
\section{Introduction}
% Simulating language emergence in deep-learning-based agent systems has recently received extensive attention from researchers.
% From the linguistic perspective, the study of emergent language may help understand the process of language evolution and test some linguistic hypotheses.
% From the AI perspective, introducing the discrete language system into the deep-learning-based agent communication scenarios is a promising way to make it more interpretable, generalizable, and human interactable.

% Lewis-style Games\cite{lewis} are widely used in many previous studies to simulate language emergence.
% This cooperation game requires two agents: the speaker and the listener. 
% In the game, the speaker produces messages to describe its private data, usually images\cite{mu2021emergent, lazaridou2017multiagent, choi2018multiagent, harding-graesser-etal-2019-emergent, dagan2021co, kottur-etal-2017-natural} or compositional symbols\cite{li2019ease, rita2022on, Ren2020Compositional, rita2022emergent} in previous studies' environments, 
% then sends them to the listener to complete discrimination or reconstruction tasks.
% When agents reach an agreement, a stable language emerges unsupervised.

% However, a critical environmental pressure was missing from the setting of previous studies: the pressure to extract abstract concepts.
% In compositional symbols environments, symbols are concepts, so there is no pressure to extract abstract concepts.
% Also, such environments are considered too simplistic to reach complex or diverse communication behaviors\cite{chaabouni2022emergent}.
% In simple image-based environments(with color, shape, style, ...), only Mu's work\cite{mu2021emergent} considers this pressure and proposes a limited solution by carefully controlling the speaker's and listener's contexts, 
% forcing the speaker to communicate the target image's most distinguishable features(they called "concepts").
% Their method does not substantially introduce the pressure to extract abstract concepts. 
% Besides, it is not extensible to more realistic natural image-based environments due to the complexity and diversity of natural images.
% Human language usually conveys abstract concepts, so it is good at expressing efficiently, generalization, and drawing inferences.
% We argue that these capabilities are also attractive and necessary for emergent languages.
% It is unlikely to emerge languages that can convey abstract concepts in these environments without the pressure to extract abstract concepts.
% A question naturally arises: can we construct a more realistic environment to study language emergence with the pressure to extract abstract concepts?

% In this work, inspired by abstract reasoning benchmarks, we propose the more realistic Reasoning Game with the reasoning pressure, forcing agents to communicate abstract rules(concepts).
% More specifically, the game's core is a cooperative reasoning task that can only be solved if the speaker communicates abstract rules implicit in his private context to guide the listener.
% For the Reasoning Game, we propose the rule-RAVEN dataset with three key designs: an easy-to-describe rule set, a rule-based candidate panels generation algorithm, and an attribute-level compositional prior.
% We also propose specialized agent architectures for the Reasoning Game and use two-stage curriculum learning techniques to ensure agents can complete the challenging game.
% Experimental results show that agents can complete the game successfully and develop a compositional language that can describe the abstract rules of reasoning problems. 
% Communicating abstract rules(concepts) is beneficial for generalizing to unseen rule combinations, 
% transferring rules from one attribute to another, and transfering to a different task setup.

%加引用
Research on emergent communication has received extensive attention in recent years due to its inspiration to the fields of linguistics and artificial intelligence.
From the linguistic perspective, the study of emergent communication may help understand the process of language evolution and test some linguistic hypotheses.
From the AI perspective, introducing discrete communication into the deep-learning-based agent system is a promising way to make it more interpretable, generalizable, and human-interactable.

%删掉一些敏感的专有名词，尽量不用abstract里没出现的名词去定义，例如private data
Lewis-style Games\cite{lewis} are widely used in many previous studies to simulate communication emergence.
This cooperation game requires two agents: the speaker and the listener. 
In the game, the speaker produces messages to describe its private data, then sends them to the listener to complete discrimination or reconstruction tasks.
When agents reach an agreement, a stable language emerges unsupervised.


However, previous attempts have hovered around emerging language under simplistic environmental settings that describe low-level perceptual features of images\cite{mu2021emergent, lazaridou2017multiagent, choi2018multiagent, harding-graesser-etal-2019-emergent, dagan2021co, kottur-etal-2017-natural} or symbols\cite{li2019ease, rita2022on, Ren2020Compositional, rita2022emergent}.
%Although an existing work\cite{mu2021emergent} tries to force agents to communicate high-level ideas by carefully controlling the speaker's and listener's context, the method essentially encourages the speaker to communicate unique human-desired low-level objects in images.
In contrast,%这里不转折，是递进 
%这里写一写后果，要能挂上communication和reasoning，最好是用引用别人的话。
%causing a enomous gap between language emergent environments and realistic human-like dialogue senarios where always reasoning and communicating high-level concepts or rules.
human language usually conveys what they think rather than what they see, so it is expressed efficiently, generalized well, and can draw reasoning.
%这句话是后果，挪到第二句，但是要找到相关的认知学文献引用，最好不是we argue...
We argue that such human-like language with high-level abstraction and complex functionalities is unlikely to emerge in the simplistic environmental settings previous studies adopted.
%写完别人在语言和AI方面的不好，这里需要一句，写communication for reasoning是high-level的，是好的。最好也有文献
%目前这句没有信息量，这句需要是一个总结性的陈述，概括一下问题，或者提一个本文的研究目标
A question naturally arises: Can we move towards the emergence of more human-like languages in realistic environmental settings?

In this work, 
%这句话能不能搞后面去，段首句还是要突出主体，前置。
%inspired by Raven's Progressive Matrix(RPM) tests, 
we propose the 
%more realistic 
Reasoning Game, encouraging agents to reason and communicate high-level rules 
%这半句可以再考虑一下要不要放在specifically后
instead of perceived low-level contexts(composed of multiple attributes).
%这里写reasoning game的定义，即让两个agent通过交流协作完成RPM问题， which is widely accepted and believed to be highly correlated with real intelligence (RAVEN论文里，找几个引用文献，real intelligence有点狂了，稍微靠点reasoning)
%这里可能有点啰嗦
Specifically, the game's core is a cooperative reasoning task, which requires the speaker to reason rules from the private context it receives and then generate language guidance to help the speaker to complete the problem it faces.
%为了能让reasoning game更XXX好，我们有两个关键的设计：1）rule-RAVEN dataset, and 2) two-stage XXX.
%对于前者, rule-RAVEN是XXX，解决了overfitting的问题。
%对于后者，two-stage的核心思路是XXX，解决了reasoning game中agent policy收敛不稳定的问题。
Moreover, we propose a symbolic dataset, rule-RAVEN, which contains several RPM problems with different rule combinations for our Reasoning Game.
The rule-RAVEN dataset is debiased by our rule-based candidate panel generation algorithm to avoid overfitting in communication.
Besides, we design a specialized agent model architecture to enable reasoning. 
We also propose a two-stage curriculum agent training method for more stable convergence in the Reasoning Game where contexts and semantics drift bilaterally.
%这里和第5章的对应关系要强一些，可以分别写两句，我们证明了XXX，后面跟一个括号（Section 5.X）
Experimental results show that, in our Reasoning Game, a semantically stable and compositional language emerges to solve reasoning problems.
The emerged language helps agents apply the extracted rules to the generalization of unseen context attributes, and to the transfer between different context attributes or even tasks.

